Zero-shot prompt-based classification: topic labeling in times of foundation models in German Tweets

Filtering and annotating textual data are routine tasks in many areas, like social media or news analytics. Automating these tasks allows to scale the analyses wrt. speed and breadth of content covered and decreases the manual effort required. Due to technical advancements in Natural Language Processing, specifically the success of large foundation models, a new tool for automating such annotation processes by using a text-to-text interface given written guidelines without providing training samples has become available. In this work, we assess these advancements in-the-wild by empirically testing them in an annotation task on German Twitter data about social and political European crises. We compare the prompt-based results with our human annotation and preceding classification approaches, including Naive Bayes and a BERT-based fine-tuning/domain adaptation pipeline. Our results show that the prompt-based approach - despite being limited by local computation resources during the model selection - is comparable with the fine-tuned BERT but without any annotated training data. Our findings emphasize the ongoing paradigm shift in the NLP landscape, i.e., the unification of downstream tasks and elimination of the need for pre-labeled training data.

==> figures/prompt.description.sentiment.tex <==
\begin{prompt}[ht]
	\begin{lstlisting}[breaklines]
prompt: str = f"""
Your task is to analyze the sentiment of the following tweet:
'''{text}'''
Thus, extract the subjective author's polarity about the tweet content and classify it into one of the following classes: {classes}
"""
	\end{lstlisting}
	\caption{description, sentiment}
	\label{prompt:description:sentiment}
\end{prompt}

==> figures/prompt.handbook.sentiment.tex <==
\begin{prompt}[ht]
	\begin{lstlisting}[breaklines]
prompt: str = f"""
Your task is to utilize the following class descriptions – label between *'s followed by its definition – to choose the one most fitting for the tweet:
*Positiv*: The tweet author's polarity towards the dominant topic is positive.
*Negativ*: The tweet author's polarity towards the dominant topic is negative.
*Neutral*: The tweet author's polarity towards the dominant topic is netural.
'''{text}'''
"""
	\end{lstlisting}
	\caption{handbook, sentiment}
	\label{prompt:handbook:sentiment}
\end{prompt}

==> figures/table.results.overview.sentiment.tex <==
\begin{table*}[ht]
	\centering
	\small
	\begin{tabular}{lr | rr | rr}
		\toprule
		& 
		\makecell[r]{\textbf{Baseline}\\Naive Bayes} & 
		\makecell[r]{\\fine-tuned} & 
		\makecell[r]{\textbf{BERT}\\w/ pre-training} & 
		\makecell[r]{\textbf{mT0}\\zero-shot} & 
		\makecell[r]{\textbf{FLAN-T5}\\zero-shot} 
		\\
		\midrule
		\textbf{negativ}   & 0.7642 & 0.7959 & \textbf{0.7768} & 0.0000 & 0.3715 \\
		\textbf{neutral}   & 0.4516 & 0.6254 & \textbf{0.6541} & 0.7089 & 0.8720 \\
		\textbf{positiv}   & 0.1923 & 0.3974 & \textbf{0.4800} & 0.0000 & 0.0000 \\
		\midrule
		\textbf{macro avg} & 0.4694 & 0.6062 & \textbf{0.6370} & 0.2363 & 0.4145 \\
		\bottomrule
	\end{tabular}
	\caption{Comparison across methods for sentiment task}
	\label{tab:results:overview:sentiment}
\end{table*}

==> figures/table.results.prompting.sentiment.tex <==
\begin{table*}[ht]
	\centering
	\small
	\begin{tabular}{lrr | rr |rr | rr}
		\toprule
		& \multicolumn{2}{c}{\textbf{base}} 
		& \multicolumn{2}{c}{\textbf{w/ task-name}} 
		& \multicolumn{2}{c}{\textbf{w/ description}} 
		& \multicolumn{2}{c}{\textbf{w/ handbook}} \\
		& \textbf{FLAN-T5} & \textbf{mT0} 
		& \textbf{FLAN-T5} & \textbf{mT0} 
		& \textbf{FLAN-T5} & \textbf{mT0} 
		& \textbf{FLAN-T5} & \textbf{mT0} \\
		\midrule
		\textbf{negativ}   & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000          & 0.0000 & 0.2885          & \textbf{0.5229} \\
		\textbf{neutral}   & 0.9864 & 0.5413 & 0.9796 & 0.6297 & \textbf{0.9932} & 0.6546 & 0.9151          & 0.0249          \\
		\textbf{positiv}   & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000          & 0.0000 & 0.0000          & 0.0000          \\
		\midrule
		\textbf{macro avg} & 0.3288 & 0.1804 & 0.3265 & 0.2099 & 0.3311          & 0.2182 & \textbf{0.4012} & 0.1826          \\
		\bottomrule
	\end{tabular}
	\caption{Comparison in prompt detail for sentiment task}
	\label{tab:results:prompting:sentiment}
\end{table*}

==> figures/table.survey.agreement.tex <==
\begin{table*}[ht]
	\centering
	\small
	\begin{tabular}{lr}
		\toprule
		                               & agreement \\
		\midrule
		\textbf{Demokratie}            & 0.5345    \\
		\textbf{Energiewende}          & 0.3662    \\
		\textbf{Migration}             & 0.6416    \\
		\textbf{Ukraineunterstützung} & 0.4587    \\
		\textbf{Wirtschaft}            & 0.3969    \\
		\midrule
		\textbf{macro avg}             & 0.4796    \\
		\bottomrule
	\end{tabular}
	\hspace{1cm}
	\begin{tabular}{lr}
		\toprule
		                   & agreement \\
		\midrule
		\textbf{negativ}   & 0.7062    \\
		\textbf{neutral}   & 0.3234    \\
		\textbf{positiv}   & 0.4242    \\
		\midrule
		\textbf{macro avg} & 0.5922    \\
		\bottomrule
	\end{tabular}
	\caption{Inter-Annotator agreement for both tasks according to Fleiss-Kappa.}
	\label{tab:survey:agreement}
\end{table*}
